Improving Language Modelling with Noise-contrastive estimation

Neural language models do not scale well when the vocabulary is large. Noise-contrastive estimation (NCE) is a sampling-based method that allows for fast learning with large vocabularies. Although NCE has shown promising performance in neural machine translation, it was considered to be an unsuccessful approach for language modelling. A sufficient investigation of the hyperparameters in the NCE-based neural language models was also missing. In this paper, we showed that NCE can be a successful approach in neural language modelling when the hyperparameters of a neural network are tuned appropriately. We introduced the 'search-then-converge' learning rate schedule for NCE and designed a heuristic that specifies how to use this schedule. The impact of the other important hyperparameters, such as the dropout rate and the weight initialisation range, was also demonstrated. We showed that appropriate tuning of NCE-based neural language models outperforms the state-of-the-art single-model methods on a popular benchmark.

==> model.tex <==
\todo[inline]{I think that explanation in the background should be improved. We can assume that people know more or less what backpropagation is and what a neural network is. Then we should provide an intuitive explanation what RNN is and then what LSTM is. At a high level. Assume that you are writing this for Alex. Then clearly define the input data tupes. I don't really understand $c_i$ right now. Note that you don't have a detailed plan for this section in the plan google doc. Perhaps you could first refine your plan in google doc, paragraph by paragraph, and then write this background section according to the detailed plan. Perhaps write backpropagation instead of BP.}

\begin{figure}[tb] %[!h]
\centering
\includegraphics[scale=0.75]{diagram_lstm_lm}
\caption{A three time step LSTM LM}
\label{diagram:lstm_lm}
\end{figure}


Theoretically, Recurrent (LSTM cell) Neural Network language model can represent a full, non-truncated context $c_i = <w_{i-1},\dots,w_1>$ for words $w_i$ using the word representation (1-to-V encoding or dense vector encoding) of the previous word $w_{i-1}$ and a continuous vector $v_{i-2}$ representing the whole previous context $c_i$. However, due to the gradient vanishing and exploding problem \cite{pmlr-v28-pascanu13}, it is not clear exactly how much previous context is actually represented by the $v_{i-2}$. %Intuitively, LSTM can store and retrieve information over long time scales using its gating mechanisms. 
Many extention the LSTM architecture, such as, Recurrent Highway Networks(RHN) \cite{DBLP:journals/corr/ZillySKS16} has been proposed to solve this long term dependency problem which would improve the language modelling performance as well. But for this paper we are not doing investigation in this direction. We will work with classic LSTM cell \cite{hochreiter1997long,gers2001long} and see how the normalisation of the output layer has impact on language modelling performance. %More specifically, we will compare between normalised and unnormalised model.  
\todo[inline]{It seems that the second part of the paragraph above could be moved to the end of section 4. In section 4 you describe methodology. In there you could say that you use state-of-the-art LSTM, but you acknowledge that improvements exist and then you mentioned a few of them. You could justify the type of LSTM that you are using, an by adding these citations you are showing that you are aware of the existing extensions.}


Unnormalised score (see $v_3$ in fig~\ref{diagram:lstm_lm}) at each time step from a LSTM cell, which does not provide any probability distribution, will be feed into a normalisation process (through softmax) as follows:

\begin{equation}
P_{LSTM}(w_i | c_i)=\frac{\exp(\theta^{\top}_{i} v_{i-1})}{\sum_{j=1}^{|V|}\exp(\theta^{\top}_{j} v_{i-1})}=\frac{\exp(\theta^{\top}_{i} v_{i-1})}{Z}
\label{eq:softmax}
\end{equation}

%\unsure{Why this latex error? comment out the following line}
Here, $P_{LSTM}(w_i | c_i)$ is the probability of word $w_i$ given context $c_i$, $\theta_{i}$ is the weight vector corresponding to the word $i$ at the output layer. $v_{i-1}$ is the recurrent vector representing the context propagated through the hidden layer, $|V|$ is the vocabulary size in the output layer. The normalising term $Z$ is known as the {\bf partition function}.

%Lets define the partition function $Z = \sum_{j=1}^{|V|}\exp(\theta^{\top}_{j} v_{i-1})$, for normalising the the probability distribution $ P_{RNN}$. 
%unnormalized score
%$$v_j = \tanh(x \times W^1) \times W_{*,j}^2$$
%for $j \in \{1, \dots, |v|\}$
% We use softmax to force a distribution. 
%$$Softmax (z_j) = \frac{\exp(z_j)}{\sum_{w \in v}{\exp(z_w)}}$$

The softmax-based RNNLM training using SGD utilising BP maximises the log likelihood or equivalently minimises the cross-entropy of the training sequence containing $N$ words. The objective is given by 

\begin{equation}
J_{SOFT}(\theta) = - \frac{1}{N} \sum_{i = 1}^{N} \ln P_{LSTM(\theta)}^{SOFT}(w_i | c_i)
\label{eq:ce_loss_softmax}
\end{equation}

So the gradient used in the optimisation for updating the $\theta$ is as follows:

\begin{equation} \label{eq:soft_ce_loss_grad}
\begin{aligned}
\frac{\partial J_{SOFT}(\theta)}{\partial \theta} & =  - \frac{1}{N} \sum_{i = 1}^{N} [ \frac{\partial (\theta_{i}^{\top} v_{i-1})}{\partial \theta}  \\  & - \sum_{j=1}^{|V|} P_{LSTM(\theta)}^{SOFT}(w_j | c_i) \frac{\partial (\theta_{j}^{\top} v_{i-1})}{\partial \theta} ]
\end{aligned}
\end{equation}

During the training of the language model this gradient computation makes the time complexity ($O(|V| \times D)$) very high. When we have a large vocabulary ($|V|$ is large), this partition function creates the performance bottleneck for training and testing phase. We dont want this expensive normalisation term. 
%\info{The rare words does not appears all the time, the gradient contribution should be handled differently from the rare words, in mini-batch how the combination of rare and frequent words make a combined contribution}. 
Noise contrastive estimation (NCE) bypass this calculation by converting this to a binary classification problem. 

In NCE, we can see the corpus as a new dataset of the following format:
 
$$((c_1,w_1), D_1)), \dots , ((c_n,w_n),D_n)$$
 
where $c$ represents the context $w_{i-n+1}, \dots, w_{i_1}$, $w_i$ represents a possible word and a random variable $D=1$ if $w_i$ is from the training corpus (true data distribution) and $D=0$ if $w_i$ is from a known chosen (known noise distribution, $P_n$) distribution. For a given context $c_i$, the NCE-based RNNLM models data samples (from corpus) as if they are generated from a mixture of two distribution ($P_{LSTM(\theta)}^{NCE}$~\footnote{assuming $P_{LSTM(\theta)}^{NCE}$ can approximate the true empirical distribution} and $P_n$) that satisfies a desired normalisation (sum-to-one constraint). Thus the requirement for the normalisation term is satisfied implicitly\todo{because ...}. In practice for LM, for each data sample, $k$ numbers of noise samples are generated, and \cite{Mnih12afast} shows that for large $k$, NCE-based parameter estimation is a close approximation of the MLE (of the data sample). The time complexity for NCE is thus $O(k \times D)$.
 
The posterior probability of a sample word generated from the $P_{LSTM(\theta)}^{NCE}$ and $P_n$ are as follows:

\begin{equation} \label{eq:posterior_p_data_p_n}
\begin{aligned}
P(D = 1| w_i , c_i) = \frac{P_{LSTM(\theta)}^{NCE}(w_i| c_i)}{P_{LSTM(\theta)}^{NCE}(w_i|c_i) + k P_n(w_i|c_i)} \\
P(D = 0| \widetilde{w_i} , c_i) = \frac{k P_n(\widetilde{w_i}|c_i)}{P_{LSTM(\theta)}^{NCE}(\widetilde{w_i}|c_i) + k P_n(\widetilde{w_i}|c_i)}
\end{aligned}
\end{equation}

Here $\widetilde{w_i}$ is a sampled word from a known distribution (for instance, uniform distribution). 

Based on this posterior distribution, the NCE minimises the following objective function,

\begin{equation} \label{eq:nce_loss}
\begin{aligned}
J_{NCE}(\theta) &= - \frac{1}{N} \sum_{i=1}^{N} [ \ln P(D = 1| w_i , c_i) \\
& + \sum_{j=1}^{k} \ln P(D = 0| \widetilde{w_{i,j}} , c_i) ]
\end{aligned}
\end{equation}

Here, for the current training word sample (from true distribution) $w_i$, there are total $k$ noise samples (from a known distribution) $\widetilde{w_{i,j}}$ were generated. For example, when $w_i = t_3$ (in fig~\ref{diagram:lstm_lm}), there can be $k$ words sampled from a uniform distribution.  

The gradient of the objective function is as follows:

\begin{equation} \label{eq:nce_loss_grad}
\begin{tiny}
\begin{aligned}
\frac{\partial J_{NCE}(\theta)}{\partial \theta} &= - \frac{1}{N} \sum_{i=1}^{N} [ \frac{k P_n (w_i|c_i)}{P_{LSTM(\theta)}^{NCE} (w_i|c_i)+k P_n(w_i|c_i)} \frac{\partial}{\partial \theta} \ln P_{LSTM(\theta)}^{NCE} (w_i|c_i) \\
& - \sum_{j=1}^{k} \frac{P_{LSTM(\theta)}^{NCE}(\widetilde{w_{i,j}}|c_i)}{P_{LSTM(\theta)}^{NCE}(\widetilde{w_{i,j}}|c_i) + k P_n(\widetilde{w_{i,j}}|c_i)} \frac{\partial}{\partial \theta} \ln  P_{LSTM(\theta)}^{NCE}(\widetilde{w_{i,j}}|c_i) ]
\end{aligned}
\end{tiny}
\end{equation}

Here, 

\begin{equation}\label{eq:P_rnn_in_nce}
\begin{aligned}
P_{LSTM(\theta)}^{NCE}(w_i | c_i) = \frac{\exp(\theta^{\top}_{i} v_{i-1})}{Z} \\
P_{LSTM(\theta)}^{NCE}(w_{i,j} | c_i) = \frac{\exp(\theta^{\top}_{j} v_{i-1})}{Z}
\end{aligned}
\end{equation}

So we still have this normalising term $Z$, but now unlike softmax, the NCE estimated distribution is not dependent on the $Z$ for normalising. In fact, $Z$ can be learnt as a parameter \cite{gutmann2010noise} or can be considered as a constant, for instance, $Z=1$ was set for all contexts in \cite{Mnih12afast,conf/emnlp/VaswaniZFC13,Zoph2016SimpleFN}.

\todo[inline]{if you could provide a detailed plan for this section in google doc, I will be able to say more. Perhaps in your NCE discussion, you could reduce the number of equations and compress the explanation to a few paragraphs where you say intuitively what is going on in NCE. I know that that's hard, but we could save some space in this way. Don't worry if you don't know how to do it now, we may need to work on this section more.} 

%The objective is based on the predicted $\hat{d}$:
 
%$$C(w) = \sum_{i}{L_{crossentropy}(d_i,\hat{d}_{i})}$$
 
%The partial derivative of the cross-entropy cost with respect to the weights.
% $$\frac{\partial C}{\partial w_j}  = \frac{1}{n} \sum_{x} x_j(\sigma(z)-y)$$

%The larger the error, the faster the neurone will learn. There are a number of modelling and experimental systems have demonstrated that better and faster learning is achieved when error is larger \cite{Kawato:1990,rumelhart1988learning}.

%https://books.google.co.uk/books?id=jMvbRFzOzHEC&pg=PA82&lpg=PA82&dq=why+large+error+leads+to+faster+learning&source=bl&ots=pKmeju50Q5&sig=XxFYDQJyF5fhV0Pu8VBTz1sxMpM&hl=en&sa=X&ved=0ahUKEwii7J3y5q7VAhWMJ8AKHbkCAlYQ6AEIHDAA#v=onepage&q=why%20large%20error%20leads%20to%20faster%20learning&f=true

%But how to use this binary classification for training LM? If we use the unnormalised score $z_j$ for the $\hat{d} = \sigma(z_j)$, then the problem is similar to softmax regression, but does not help in training LM.

%To solve this problem,  a new random variable $D$ is being introduced. For true sample $D=1$, for $D=0$ produce a sample from a noise distribution. In practice, for each true sample there will be $k$ noise samples. For the forward pass scores for $k+1$ words will be calculated. This involves extracting $k+1$ rows from the $V \times D$ decoding matrix in the output layer, multiplying the D dimensional internal representation with the $(k+1) \times D$ matrix. 

%$$z_j = \sigma(\sum_{i =1}^{D} w_{i,j} h_i)$$

%Here $h_i$ is the output of the last hidden layer. 





==> reguraliser.tex <==
To avoid overfitting, dropout \cite{srivastava2014dropout} was used on non-recurrent nodes as a regulariser \cite{zaremba2014recurrent}. %For small dataset like PTB, regularisation is even more important. 
We have seen that for large models where softmax overfits even after using dropout, NCE can be used with smaller dropout rate and does not get overfitted so easily. Consequently, with the same dataset NCE can give better generalisation as we get smaller test PPL.\todo{It seems to me that everything after the first sentence should be moved to the description of results. It is just part of the description of the results. What do you think? Is there any methodological guidance here that we want explain to other people? If not so, we may want to remove this sub-section.Ans: Methodologically, for large model we have used less dropout rate for NCE and it gave better generalisation. For medium model, the dropout rate was same for NCE and softmax. We need regulariser(dropout) more for large model. But we can remove this subsection}

==> sampling_techniques.tex <==
%Noise contrastive estimation (NCE) replaces the expensive vocabulary-sized softmax operation at the final layer of language models with a cheaper sampling-based operation, which results in significant speed-up during training. 
%\info{Commented out paragraph}
For NCE, noise distribution plays an important rule. The proposed model is depend on the noise sample generated from a known distribution to contrast the original data samples. For example, for language model, sampling the contrastive word class from uniform distribution and unigram distribution is not the same. Intuitively for a good training noise distribution should be close to the data distribution \cite{gutmann2010noise}. As we dont know the data distribution, it is very difficult to design a noise distribution that is a good match with the data distribution. For language modelling, one can assume that sampling from n-gram model ($n \ge 5$) with Kneser Ney smoothing would give good representation of the noise distribution. Although according to \cite{bengio2008adaptive}, neural  language  models  and n-gram  models  learn very different distributions. Moreover, for this experiment we intend to utilise the advancement of GPU technology for time efficient computation. Since we typically sample different noise samples for each training instance, the gradient computations for the NCE objective are not manageable to dense matrix operations, making it difficult to benefit from fast dense matrix arithmetic on GPUs. So following \cite{Zoph2016SimpleFN}, we have used sharing of the noise samples across all the training instances in a mini-batch. Sharing noise samples allows us to describe NCE gradients with dense matrix operations, and implement them easily on the GPU. Because of that we have to come up with a noise sample that describe best characteristic of the word distribution. As word distribution follows Zipf's law \cite{Piantadosi2014}, we have used noise samples from Zipfian (log-uniform) distribution. To be able to use sample from that distribution the words in the vocabulary has to be sorted in the descending order of the frequency( tensorflow requirement). %There are other noise samples can be utilised, such as unigram distribution. Unigram distribution is similar to the zipfian distribution when sorted in descending order, and both are based on the frequency of the words. 

%The base distribution for this operation in tensorflow is an approximately log-uniform or Zipfian distribution: 
%\begin{equation}
%\begin{aligned}
%P(class) = \frac{(\log(class + 2) - \log(class + 1))}{\log(range_{max} + 1)}
%\end{aligned}
%\end{equation}

%If NCE is need to be used in a situation where this is not possible (for example the vocabulary is not fixed) then, other noise distribution has to be utilised. 

There are other noise samples can be utilised, such as unigram distribution. Unigram distribution is similar to the zipfian distribution as both are the based on the frequency of the words. 
%\info{Commented out paragraph}
We have also proposed a noise distribution criteria where the words do not required to be sorted in any order. The proposed distribution is based on the hypothesis that words that have appeared in more contexts in the past are more likely to appear in some new context as well. Kneser-Ney Smoothing for n-gram is also based on the same hypothesis. The difference is we are not using this hypothesis for smoothing rather for designing noise distribution. We have defined left context and both context based word distribution. For left context based distribution, the frequency of each word was counted according to the number of distinct left context in the corpus. For both context based word distribution, the distribution is based on the number of distinct left and right context of the word in the corpus. We have also used uniform distribution for comparison where none of the noise distribution described above is not applicable.



%open vocabulary
%https://openreview.net/pdf?id=SygGlIBcel

